SONAR: Sentence-Level Multimodal and Language-Agnostic Representations

We introduce SONAR, a new multilingual and multimodal fixed-size sentence embedding space. Our single text encoder, covering 200 languages, substantially outperforms existing sentence embeddings such as LASER3 and LabSE on the xsim and xsim++ multilingual similarity search tasks. Speech segments can be embedded in the same SONAR embedding space using language-specific speech encoders trained in a teacher-student setting on speech transcription data. Our encoders outperform existing speech encoders on similarity search tasks. We also provide a text decoder for 200 languages, which allows us to perform text-to-text and speech-to-text machine translation, including for zero-shot language and modality combinations. Our text-to-text results are competitive compared to the state-of-the-art NLLB~1B model, despite the fixed-size bottleneck representation. Our zero-shot speech-to-text translation results compare favorably with strong supervised baselines such as Whisper.

==> SpeechMine_tab.tex <==

\begin{tabular}[t]{@{}ll|r|rr@{}} \\
\toprule
%\multirow{2}{*}{\bf ISO} & \multirow{2}{*}{\bf Language}  & \bf Train & \bf Decode & \bf Whisper  \\
% & & \textrm{audio [h]}  & \textrm{BLEU13} & \bf BLEU13a  \\
 ISO & Language & Train & Ours & Whisper \\
\midrule
\textrm{arb}  & \textrm{MS Arabic} & {822} & {28.7} & {25.5}\\
\textrm{ben}  & \textrm{Bengali} & {335} & {18.9} & {13.2}\\
\textrm{cat}  & \textrm{Catalan} & {1738} & {35.1} & {34.2}\\
\textrm{cmn}  & \textrm{Mandarin Chinese} & {9320} & {16.2} & {18.4}\\
\textrm{ces}  & \textrm{Czech} & {181} & {29.3} & {27.8}\\
\textrm{cym}  & \textrm{Welsh} & {99} & {14.5} & {13.0}\\
\textrm{dan}  & \textrm{Danish} & {115} & {31.9} & {32.7}\\
\textrm{deu}  & \textrm{German} & {3329} & {32.7} & {34.6}\\
\textrm{est}  & \textrm{Estonian} & {131} & {23.8} & {18.7}\\
\textrm{fin}  & \textrm{Finish} & {184} & {22.2} & {22.1}\\
\textrm{fra}  & \textrm{French} & {2057} & {31.2} & {32.2}\\
\textrm{hin}  & \textrm{Hindi} & {150} & {19.2} & {22.0}\\
\textrm{ind}  & \textrm{Indonesian} & {269} & {26.5} & {29.1}\\
\textrm{ita}  & \textrm{Italian} & {588} & {25.3} & {23.6}\\
\textrm{jpn}  & \textrm{Japanese} & {17319} & {17.4} & {18.9}\\
\textrm{kan}  & \textrm{Kannada} & {114} & {20.0} & {11.6}\\
\textrm{kor}  & \textrm{Korean} & {316} & {15.0} & {21.3}\\
\textrm{mlt}  & \textrm{Maltese} & {106} & {23.3} & {13.5}\\
\textrm{nld}  & \textrm{Dutch} & {1723} & {25.5} & {24.0}\\
\textrm{pes}  & \textrm{Western Persian} & {386} & {22.3} & {19.6}\\
\textrm{por}  & \textrm{Portuguese} & {269} & {35.4} & {38.1}\\
\textrm{pol}  & \textrm{Polish} & {304} & {21.1} & {22.3}\\
\textrm{ron}  & \textrm{Romanian} & {135} & {32.1} & {31.5}\\
\textrm{rus}  & \textrm{Russian} & {259} & {25.4} & {27.8}\\
\textrm{slk}  & \textrm{Slovak} & {102} & {29.5} & {26.1}\\
\textrm{spa}  & \textrm{Spanish} & {1511} & {24.3} & {23.3}\\
\textrm{slv}  & \textrm{Slovenian} & {65} & {23.6} & {17.0}\\
\textrm{swh}  & \textrm{Swahili} & {361} & {22.6} & { 7.2}\\
\textrm{tam}  & \textrm{Tamil} & {245} & {14.3} & { 9.2}\\
\textrm{tel}  & \textrm{Telugu} & {84} & {15.8} & {12.5}\\
\textrm{tgl}  & \textrm{Tagalog} & {108} & {13.3} & {24.4}\\
\textrm{tha}  & \textrm{Thai} & {195} & {15.3} & {16.1}\\
\textrm{tur}  & \textrm{Turkish} & {174} & {21.0} & {26.6}\\
\textrm{ukr}  & \textrm{Ukrainian} & {105} & {28.0} & {29.4}\\
\textrm{urd}  & \textrm{Urdu} & {185} & {17.6} & {17.2}\\
\textrm{uzn}  & \textrm{Uzbek} & {115} & {17.9} & { 6.0}\\
\textrm{vie}  & \textrm{Vietnamese} & {194} & {17.8} & {20.4}\\
\midrule
\multicolumn{2}{l}{\textrm{Total/avg}} & {43693} & {23.1} & {21.9}\\
\bottomrule
\end{tabular}

